Progressive Volume Distillation with Active Learning for Efficient NeRF Architecture Conversion

Neural Radiance Fields (NeRF) have been widely adopted as practical and versatile representations for 3D scenes, facilitating various downstream tasks. However, different architectures, including the plain Multi-Layer Perceptron (MLP), Tensors, low-rank Tensors, Hashtables, and their combinations, entail distinct trade-offs. For instance, representations based on Hashtables enable faster rendering but lack clear geometric meaning, thereby posing challenges for spatial-relation-aware editing. To address this limitation and maximize the potential of each architecture, we propose Progressive Volume Distillation with Active Learning (PVD-AL), a systematic distillation method that enables any-to-any conversion between diverse architectures. PVD-AL decomposes each structure into two parts and progressively performs distillation from shallower to deeper volume representation, leveraging effective information retrieved from the rendering process. Additionally, a three-level active learning technique provides continuous feedback from teacher to student during the distillation process, achieving high-performance outcomes. Experimental evidence showcases the effectiveness of our method across multiple benchmark datasets. For instance, PVD-AL can distill an MLP-based model from a Hashtables-based model at a 10~20X faster speed and 0.8dB~2dB higher PSNR than training the MLP-based model from scratch. Moreover, PVD-AL permits the fusion of diverse features among distinct structures, enabling models with multiple editing properties and providing a more efficient model to meet real-time requirements like mobile devices. Project website: https://sk-fun.fun/PVD-AL.

==> tables/models.tex <==

    \begin{tabular}{ll}
    \toprule
    TensoRF [10] & Gaussian-splatting [12] \\
    \midrule
    Replace Objects [10, 35] & Remove Objects [10, 35] \\
    Image Question Answering [23] & Super-resolution [60] \\
    Image-to-Text [23] & Text-to-Image [35] \\
    Image-to-Edge [45] & Edge-to-Image [53] \\
    Image-to-Line [16] & Line-to-Image [53] \\
    Image-to-Hed [44] & Hed-to-Image [53] \\
    Image-to-Seg [24] & Seg-to-Image [53] \\
    Image-to-Depth [34, 33] & Depth-to-Image [53] \\
    Image-to-NormalMap [34, 33] & NormalMap-to-Image [53] \\
    Image-to-Sketch [44] & Sketch-to-Image [53] \\
    Image-to-Pose [6] & Pose-to-Image [53] \\
    Text-driven Stylize [15] & Image-driven Stylize [16] \\
    \bottomrule
    \end{tabular}%


